Future Aware Safe Active Learning of Time Varying Systems using Gaussian Processes

Experimental exploration of high-cost systems with safety constraints, common in engineering applications, is a challenging endeavor. Data-driven models offer a promising solution, but acquiring the requisite data remains expensive and is potentially unsafe. Safe active learning techniques prove essential, enabling the learning of high-quality models with minimal expensive data points and high safety. This paper introduces a safe active learning framework tailored for time-varying systems, addressing drift, seasonal changes, and complexities due to dynamic behavior. The proposed Time-aware Integrated Mean Squared Prediction Error (T-IMSPE) method minimizes posterior variance over current and future states, optimizing information gathering also in the time domain. Empirical results highlight T-IMSPE's advantages in model quality through toy and real-world examples. State of the art Gaussian processes are compatible with T-IMSPE. Our theoretical contributions include a clear delineation which Gaussian process kernels, domains, and weighting measures are suitable for T-IMSPE and even beyond for its non-time aware predecessor IMSPE.

==> figures/figure_drift_NLL.tex <==


\begin{figure}[tb]

\centering

\begin{tikzpicture}

\pgfplotstableread[col sep=comma]{data_drift_NLL.csv}\csvdata
\pgfplotstabletranspose\datatransposed{\csvdata} 

\begin{axis}[
    axis lines=middle,
    xmin=0, xmax=10.5,
    ymin=-1.1, ymax=5.1,
    ytick={-1,0.0,1.0,2.0,3.0,4.0,5.0},
    yticklabels={-1,0.0,1.0,2.0,3.0,4.0,5.0},
    ylabel = {NLL/data},
    xtick={0,5,10},
    xticklabels={0,50,100},
    xlabel = {steps},
    legend style={at={(0.6,0.25)},anchor=north}
]

\addplot[draw=red] table[x index=1,y index=6] {\datatransposed};
\addlegendentry{entropy}

\addplot[draw=blue] table[x index=1,y index=3] {\datatransposed};
\addlegendentry{T-IMSPE (ours)}


\addplot[draw=red,dotted] table[x index=1,y index=5] {\datatransposed};

\addplot[draw=red,dotted] table[x index=1,y index=7] {\datatransposed};

\addplot[draw=blue,dotted] table[x index=1,y index=2] {\datatransposed};

\addplot[draw=blue,dotted] table[x index=1,y index=4] {\datatransposed};


\end{axis}

\end{tikzpicture}

\caption{%
    This diagram shows the negative log likelihood (NLL) drift experiment from Subsection~\ref{subsection_drift}.
    Due to the high drift, the NLL increases non-monotonically for both Entropy (red) and T-IMSPE (blue).
    In contrast to the RMSE from Figure~\ref{figure_drift_RMSE} and Figure~\ref{figure_drift_RMSE_gain}, entropy is superior to T-IMSPE, both on average and also the $1\sigma$ confidence intervals.
    We interpret this as more suitable hyperparameters being learned by entropy, which leads to better variance predictions, whereas T-IMSPE results in better mean predictions despite suboptimal hyperparameters.
    The NLL is plotted in the convention of GPyTorch, where we do not show the actual NLL, but the NLL divided by the number of validation data points.}
\label{figure_drift_NLL}

\end{figure}
